How Can Context Help? Exploring Joint Retrieval of Passage and Personalized Context

The integration of external personalized context information into document-grounded conversational systems has significant potential business value, but has not been well-studied. Motivated by the concept of personalized context-aware document-grounded conversational systems, we introduce the task of context-aware passage retrieval. We also construct a dataset specifically curated for this purpose. We describe multiple baseline systems to address this task, and propose a novel approach, Personalized Context-Aware Search (PCAS), that effectively harnesses contextual information during passage retrieval. Experimental evaluations conducted on multiple popular dense retrieval systems demonstrate that our proposed approach not only outperforms the baselines in retrieving the most relevant passage but also excels at identifying the pertinent context among all the available contexts. We envision that our contributions will serve as a catalyst for inspiring future research endeavors in this promising direction.

==> 3-dataset-WOO.tex <==
\subsection{Wizard-of-Oz Approach}

The first approach is the classical wizard-of-oz setting where two humans chat with each other. The agent role has access to document while the user role does not.
Before engaging two humans into conversation, besides the seed intent, we also provide the persona and context. To simulate real-world scenarios, we sample from a set of persona and context that is consistent with the seed intent.

\begin{description}[style=unboxed,leftmargin=0cm]
    
\item[Persona and context]

First, we crowd-source the relevant subset of attributes and value constraints/conditions associated with each document.
(Nice to have: use a tool to mark conditions in documents to help annotators.)

Then, we developed an algorithm to \hwan{Hui}
1) aggregate the whole set of attributes and value ranges; and 
2) sample persona and context with constraints/conditions and distributions.

\item[Initial intent] is crowd-sourced in a similar way.


\item[Dialogue with grounding document] Multi-turn conversations are curated in the classical wizard-of-oz way, where each initial intent is assigned a sampled user persona and context that is consistent with the intent. During the conversation, the agent role has access to relevant pieces of document and marks the piece of document (if any) being used. Both the agent and the user roles are asked to converse with the user persona and context in mind.

\end{description}

Please refer to Appendix for more details on the design and guideline of the data collection process.

